Learning Deep Structured Models

Many problems in real-world applications involve predicting several random variables which are statistically related. Markov random fields (MRFs) are a great mathematical tool to encode such relationships. The goal of this paper is to combine MRFs with deep learning algorithms to estimate complex representations while taking into account the dependencies between the output random variables. Towards this goal, we propose a training algorithm that is able to learn structured models jointly with deep features that form the MRF potentials. Our approach is efficient as it blends learning and inference and makes use of GPU acceleration. We demonstrate the effectiveness of our algorithm in the tasks of predicting words from noisy images, as well as multi-class classification of Flickr photographs. We show that joint learning of the deep features and the MRF parameters results in significant performance gains.

==> approach.tex <==
\section{Non-linear Structured Prediction}

%{\color{red} Add one or two sentences saying what the section is going to be}
In this section we define non-linear structured prediction more formally and derive an efficient message passing algorithm which blends learning and inference.
To this end let $y\in\Y$ be the set of random variables we are interested in predicting, with $y = (y_1, \ldots, y_N)$. % \eg, the pixels in the image or the words in a sentence.  
In this work we assume the space of valid configurations to be a product space, \ie, $\Y = \prod_{i=1}^N \Y_i$, and the domain of each individual variable $y_i$ to be  discrete, \ie,   $\Y_i = \{1, \ldots, |\Y_i|\}$.

Given  input data $x\in\X$ and  parameters $w\in\mathbb{R}^A$ of the scoring function $F(x,y;w) : \X\times\Y\times\mathbb{R}^A \rightarrow \mathbb{R}$, inference amounts to finding the highest scoring  configuration $y^\ast$: %{\color{red} I don't like A as a dimensionality. Can we use D or something else} {\color{blue} tradition is $F$ which doesn't work anymore; I thought $D$ was to similar to $\D$; other suggestions ;)}
\[
  y^* = \arg \max_{y} F(x,y;w).
\]
Log-linear models are a special case of this function, with  $F(x,y;w) = w^\top \phi(x,y)$. In this setting CRFs~\cite{Lafferty2001}, structured Support Vector Machines~\cite{Taskar2003,Tsochantaridis2005} or interpolations of those~\cite{Hazan2010b} are typically employed to learn the linear weights $w$. %{\color{red} talk here about CRFs and SSVM} 

In this work, we consider the more general setting in which $F(x,y;w)$ may be non-linear and non-concave in $w$. Towards this goal, we extend the structured prediction framework of~\cite{Hazan2010b} to non-linear functions. 
%Importantly we assume the optimum to be well defined. {\color{red} I did not underatnd what you mean here so I remove}
During learning we are interested in  finding the parameters $w$ of our model, given a training set $\D$ of input-output pairs $(x,y)\in\D$.  We let the probability of an arbitrary configuration $\hat y$ be given by the loss augmented likelihood
\[
  p_{(x,y)}(\hat{y} | w,\epsilon) = \frac{1}{Z_\epsilon(x,y,w)} \exp(F(x,\hat{y};w) + \ell(y,\hat{y}))^{1/\epsilon}.
\]
Hereby $\ell(y,\hat{y}) : \Y\times\Y \rightarrow \mathbb{R}^+\cup\{0\}$ denotes the loss function which compares a prediction $\hat y$ with a ground truth label $y$, and $Z_\epsilon(x,y,w)$ refers to the partition function, normalizing the distribution $p_{(x,y)}$ to lie within the probability simplex $\Delta$ via $Z(x,y,w) = \sum_{\hat y \in \Y} \exp \left(F(x,\hat y;w) + \ell(y,\hat y) \right)^{1/\epsilon}$. The temperature parameter $\epsilon \geq 0$ is used to adjust the uniformity of the distribution.

The learning task is defined as minimizing the negative log-likelihood $-\ln p_{(x,y)}(y|w,\epsilon)$ of the training data $\D$ \wrt $w$, \ie, 
\be
  \min_{w} \sum_{(x,y) \in \D}\left(\epsilon\ln Z_\epsilon(x,y,w) - F(x,y;w) \right).
	\label{eq:Learning}
\ee
%Note that we assumed $\ell(y,y) \equiv 0$ $\forall y\in\Y$.

%We extend the log partition function by introducing a temperature parameter $\epsilon$ \cite{hazan2010primal} as follows.
%\begin{align}
  %\label{eqn:struct_pred_prog}
  %\min_{w} \sum_{(x,y) \in \D}\left(\epsilon\ln Z_{\epsilon}(x,y,w) - F(x,y;w) \right)
%\end{align}
%where $\epsilon\ln Z_{\epsilon}(x,y,w) = \epsilon \ln \sum_{\hat{y} \in \mathcal{Y}} \exp \left( \frac{F(x,\hat{y};w) + \ell(y,\hat{y})}{\epsilon} \right)$

Subsequently we make use of the relationship between the scaled log-partition function $\epsilon \ln Z_\epsilon$ and the maximum of the negative Gibbs-Helmholtz free energy~\cite{Wainwright2008,Koller2009}, \ie, expectation plus entropy $H$, which is summarized in the following lemma (with a proof sketch given for completeness). 
\begin{lemma}
\label{lem:LogPartHelm}
The log-partition function is the maximum of the negative Gibbs-Helmholtz free energy:
\begin{align}
  \label{eqn:log_partition}
  \epsilon\ln Z_{\epsilon}(x,y,w) = \max_{p_{(x,y)}(\hat{y}) \in \Delta} \sum_{\hat{y} \in \mathcal{Y}} p_{(x,y)}(\hat{y}) \Big(F(x,\hat{y};w) + \ell(y,\hat{y}) \Big) + \epsilon H(p_{(x,y)}).
\end{align}
\end{lemma}
{\bf Proof:} Either via conjugate duality or by noting that the minimum of the Kullback-Leibler divergence equals zero, \ie, $\min_{p_{(x,y)}\in\Delta} D_{\operatorname{KL}}\left(p_{(x,y)} \mid \frac{1}{Z_\epsilon}\exp\left(F(x,\hat y;w) + \ell(y,\hat y)\right)\right) = 0$. \hfill$\blacksquare$
%{\color{blue} Maybe put this as a small lemma} We know that the log partition function is the conjugate dual of the entropy (SHOWN BY KL DIVERGENCE?), i.e.,


For many applications, our model $F(x,y;w)$ as well as the employed loss $\ell(y,\hat y)$ decompose into a sum of functions, each depending on a local subset of variables $y_r$, \ie,
%\[
%  F(x,y;w) = \sum_k f_k(x,y;w_k) = \sum_k \big(  \sum_{r \in \mathcal{V}_k} f_{k,i}(x,y_i;w_k) + \sum_{\alpha \in \mathcal{E}_k} f_{k,\alpha}(x,y_\alpha;w_k) \big)
%\]
\[
  F(x,y;w) = \sum_{r\in\R} f_r(x,y_r;w) \quad\text{and}\quad \ell(y,\hat{y}) = \sum_{r\in\R} \ell(y,\hat y_r),
\]
where $r$ is a restriction of the variable tuple $y = (y_1, \ldots, y_N)$ to the subset $r\subseteq\{1, \ldots, N\}$, more formally $y_r = (y_i)_{i\in r}$. All subsets $r$ required to compute the model function $F$ and the loss $\ell$ are summarized in the set $\R$.
%{\color{red} shouldn't we have defined two different sets of regions? Or at least say that for convenience we use the same R and this is the union of regions? or something? Make it a bit more splicit}
%so is the loss function:
%\[
%  \ell(y,\hat{y}) = \sum_{i \in \mathcal{V}} \ell(y_i, \hat{y}_i) + \sum_{\alpha \in \mathcal{E}} \ell(y_\alpha,\hat{y}_\alpha)
%\]
%\[
  %\ell(y,\hat{y}) = \sum_r\ell(y,\hat y_r)
%\]


Plugging this decomposition into  \equref{eqn:log_partition}, we obtain the scaled log-partition function 
%\begin{align}
  %\label{eqn:log_partition_local}
  %\ln Z_{\epsilon}(x,y) = \max_{p(\hat{y}) \in \Delta} \sum_{i, \hat{y}_i} p_i(\hat{y}_i) \Big(\ell(y_i,\hat{y}_i) + \sum_{k:i \in \mathcal{V}_k}f_{k,i}(x,\hat{y}_i;w_k) \Big) +  \sum_{\alpha, \hat{y}_\alpha} p_\alpha(\hat{y}_\alpha) \Big(\ell(y_\alpha,\hat{y}_\alpha) + \sum_{k:\alpha \in \mathcal{E}_k}f_{k,\alpha}(x,\hat{y}_\alpha;w_k) \Big) + \epsilon H(\boldsymbol{p})
%\end{align}
%\begin{align}
  %\label{eqn:log_partition_local}
  %\epsilon\ln Z_{\epsilon}(x,y,w) = \max_{p_{(x,y)}(\hat{y}) \in \Delta} \sum_{\hat y} p_{(x,y)}(\hat y)\left(\sum_r f_r(x,\hat y_r;w) + \ell_r(y,\hat y_r)\right) + \epsilon H(p_{(x,y)})
%\end{align}
%which is the same as
\bes
\epsilon\ln Z_\epsilon(x,y,w) = \max_{p_{(x,y)}(\hat y) \in \Delta}\sum_{r,\hat y_r} p_{(x,y),r}(\hat y_r)f_r^\ell(x,\hat y_r;w) + \epsilon H(p_{(x,y)}),
\ees
where we have introduced  marginals $p_{(x,y),r}(\hat y_r) = \sum_{y\setminus y_r} p_{(x,y)}(y)$ and the loss augmented function  $f_r^\ell(x,\hat y_r;w) = f_r(x,\hat y_r;w) + \ell_r(y,\hat y_r)$.

Despite the locality of both the scoring function and the loss, the learning task specified in \equref{eq:Learning} remains computationally challenging since the entropy $H(p_{(x,y)})$ can only be computed exactly for a small set of models of interest. In addition, the marginalization constraints are generally exponential in size. %This is intractable because of entropy over joint, \ie,  and because of marginalization constraints, \ie, $p_{(x,y),r}$ are required to be the true marginals of $p_{(x,y)}$.
To deal with both issues we approximate the true marginals $p_{(x,y),r}$ with local beliefs $b_{(x,y),r}$ that are not required to fulfill marginalization constraints globally, but only locally,  \ie, marginals $b_{(x,y),r}$ are not required to arise from a common joint distribution $p_{(x,y)}$~\cite{Wainwright2008}. In addition, we approximate the entropy via the fractional entropy~\cite{Wiegerinck2003}, \ie, $H(p_{(x,y)}) \approx \sum_r c_r H(b_{(x,y),r})$, which employs counting numbers $c_r$ to weight the marginal entropy contributions. Putting all this together,  our approximation reads as follows: %{\color{red} do you need to say for all x,y? That's bizarre here. Isn't the for all implicit when you have the equality?}
\bea
\epsilon\ln Z_\epsilon(x,y,w) \approx \max_{b_{(x,y)}} && \hspace{-0.5cm}\sum_{r,\hat y_r} b_{(x,y),r}(\hat y_r)f_r^\ell(x,\hat y_r;w) + \sum_r \epsilon c_r H(b_{(x,y),r}) \label{eq:approxInf}\\
\text{s.t.}&& \hspace{-0.5cm}b_{(x,y)}\in\mathcal{C}_{(x,y)} = \left\{\hspace{-0.2cm}\barr{ll}\forall r & \hspace{-0.2cm}b_{(x,y),r}\in\Delta\\\forall r,\hat y_r,p\in P(r) & \hspace{-0.2cm}\sum_{\hat y_p\setminus \hat y_r} b_{(x,y),p}(\hat y_p) = b_{(x,y),r}(\hat y_r),\earr\right.\nonumber
\eea
where $P(r)$ refers to the set of parents of region $r$, \ie, $P(r) \subseteq \{p\in\R : r \subset p\}$, which subsumes those regions for which we want the marginalization constraint to hold. Conversely, we define the set of children $C(r) = \{c\in\R : r\in P(c)\}$. %{\color{red} say once sentence what they are?}.

%Equation \ref{eqn:log_partition_local} can be approximated by (1) replacing the marginal probabilities $p_i(\hat{y}_i)$ and $p_\alpha(\hat{y}_\alpha)$ with beliefs $b_i(\hat{y}_i)$ and $b_\alpha(\hat{y}_\alpha)$, and (2) decomposing the entropy term into sum of local entropies. Then, we have
%\begin{align}
  %\label{eqn:log_partition_approx}
  %\ln Z_{\epsilon}(x,y) \approx & \max_{b_i,b_\alpha} \sum_{i, \hat{y}_i} b_i(\hat{y}_i) f_{(x,y),i}(\hat{y}_i;w)  +  \sum_{\alpha, \hat{y}_\alpha} b_\alpha(\hat{y}_\alpha) f_{(x,y),\alpha}(\hat{y}_\alpha;w)  + \epsilon \Big( \sum_i c_i H(b_i) + \sum_\alpha c_\alpha H(b_\alpha) \Big) \\
                         %& s.t. \ \ \ b_i(\hat{y}_i) \in \Delta_i, \ b_\alpha(\hat{y}_\alpha) \in \Delta_\alpha, \ \sum_{\hat{y}_\alpha \setminus \hat{y}_i}b_\alpha(\hat{y}_\alpha) = b_i(\hat{y}_i)  \nonumber
%\end{align}
%where $f_{(x,y),i}(\hat{y}_i;w) \equiv \Big(\ell(y_i,\hat{y}_i) + \sum_{k:i \in \mathcal{V}_k}f_{k,i}(x,\hat{y}_i;w_k) \Big)$, $f_{(x,y),\alpha}(\hat{y}_\alpha;w) \equiv \Big(\ell(y_\alpha,\hat{y}_\alpha) + \sum_{k:\alpha \in \mathcal{E}_k}f_{k,\alpha}(x,\hat{y}_\alpha;w_k) \Big)$, and $c_i$, $c_\alpha$ are the counting numbers.

Given the  approximation of the scaled partition function defined in \equref{eq:approxInf} we learn the parameters of the non-linear model $w$ by solving the following program:
\be
\min_w \!\!\sum_{(x,y)\in\D}\!\! \left(\max_{b_{(x,y)}\in\mathcal{C}_{(x,y)}} \!\!\left\{\sum_{r,\hat y_r} b_{(x,y),r}(\hat y_r)f_r^\ell(x,\hat y_r;w) + \sum_r\epsilon c_r H(b_{(x,y),r})\!\!\right\} \!-\! F(x,y;w)\!\!\right).
\label{eq:structPredGeneral}
\ee

For general counting numbers we have to solve the maximization \wrt beliefs $b$ exactly to obtain a subgradient \wrt $w$.  We can however derive a more efficient algorithm by blending minimization \wrt $w$ and maximization of the beliefs $b$ when all counting numbers are positive. To interleave both programs  we convert maximization of the beliefs into a minimization by dualizing \wrt $b$. This can be done since the maximization problem is concave in $b_{(x,y)}$ if $\forall r$, $c_r \geq 0$. Note that we assumed $\epsilon \geq 0$ throughout. %{\color{red} shouldn't' we talk about positive $\epsilon$?}

\begin{claim}
Assume $c_r \geq 0$ $\forall r$ and let $\overline{F}(w) = \sum_{(x,y)\in\D} F(x,y;w)$ denote the sum of empirical function observations. %{\color{red} empirical model is a weird term}
Let  $\lambda_{(x,y),r\rightarrow p}(\hat y_r)$ be the Lagrange multipliers for each marginalization constraint $\sum_{\hat y_p\setminus\hat y_r} b_{(x,y),p}(\hat y_p) = b_{(x,y),r}(\hat y_r)$ within $\C_{(x,y)}$ defined in \equref{eq:approxInf}. Then the approximated general structured prediction task given in \equref{eq:structPredGeneral} is equivalently given via: %{\color{red} shouldn't' we talk about positive $\epsilon$?}
\be
\min_{w,\lambda} \sum_{(x,y),r} \epsilon c_r \ln\sum_{\hat y_r}\exp\frac{f_r^\ell(x,\hat y_r;w) + \!\!\sum\limits_{c\in C(r)}\!\!\lambda_{(x,y),c\rightarrow r}(\hat y_c) - \!\!\sum\limits_{p\in P(r)}\!\! \lambda_{(x,y),r\rightarrow p}(\hat y_r)}{\epsilon c_r} - \overline{F}(w).
\label{eq:structPredGeneralDual}
\ee
\end{claim}
\vspace{-0.3cm}
{\bf Proof:} To obtain the dual of the maximization \wrt $b_{(x,y)}$ we utilize its Lagrangian 
\bes
L_{(x,y)} %&=& \sum_{r,\hat y_r} \left(f_r(x,\hat y_r;w) + \ell_r(y,\hat y_r)\right) + \sum_r \epsilon c_r H(b_{(x,y),r}) + \sum_{r,\hat y_r,p\in P(r)} \lambda_{(x,y),r\rightarrow p}(\hat y_r)\left(\sum_{\hat y_p\setminus \hat y_r} b_p(\hat y_p) - b_r(\hat y_r)\right)\\
= \sum_{r,\hat y_r} b_{(x,y),r}(\hat y_r)\!\left(\!\!f_r^\ell(x,\hat y_r;w) + \!\!\!\sum_{c\in C(r)}\!\!\!\lambda_{(x,y),c\rightarrow r}(\hat y_c) - \!\!\!\sum_{p\in P(r)}\!\!\! \lambda_{(x,y),r\rightarrow p}(\hat y_r)\!\!\right)\! + \sum_{r}\epsilon c_r H(b_{(x,y),r}).
\ees
Maximization of the Lagrangian \wrt the primal variables $b$ is possible via \lemref{lem:LogPartHelm} and we obtain the dual function being the first term in \equref{eq:structPredGeneralDual}.
%\bes
%\max_b L_{(x,y)}() = \sum_r \epsilon c_r \ln\sum_{\hat y_r}\exp\frac{f_r(x,\hat y_r;w) + \ell_r(y,\hat y_r) + \sum_{c\in C(r)}\lambda_{(x,y),c\rightarrow r}(\hat y_c) - \sum_{p\in P(r)} \lambda_{(x,y),r\rightarrow p}(\hat y_r)}{\epsilon c_r}
%\ees
For strict convexity, \ie, $\epsilon c_r > 0$ we reconstruct the beliefs to be proportional to the exponentiated, loss-augmented re-parameterization score %$\left(f_r^\ell(x,\hat y_r;w) + \sum_{c\in C(r)}\lambda_{(x,y),c\rightarrow r}(\hat y_c) - \sum_{p\in P(r)} \lambda_{(x,y),r\rightarrow p}(\hat y_r)\right)/(\epsilon c_r)$, \ie,
\bes
b_{(x,y),r} \propto \exp \frac{f_r^\ell(x,\hat y_r;w) + \sum_{c\in C(r)}\lambda_{(x,y),c\rightarrow r}(\hat y_c) - \sum_{p\in P(r)} \lambda_{(x,y),r\rightarrow p}(\hat y_r)}{\epsilon c_r}.
\ees
For $\epsilon c_r = 0$ the beliefs correspond to a uniform distribution over the set of maximizers of the loss-augmented re-parameterization score, which concludes the proof. \hfill$\blacksquare$



%We introduce Lagrange multipliers $\lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)$ for every marginalization constraint $\sum_{\hat{y}_\alpha \setminus \hat{y}_i}b_\alpha(\hat{y}_\alpha) = b_i(\hat{y}_i)$, and the Lagrangian of Equation \ref{eqn:log_partition_approx} is:
%\begin{align}
   %L(b_i,b_\alpha,\lambda;w) = \sum_{i, \hat{y}_i} b_i(\hat{y}_i) f_{(x,y),i}(\hat{y}_i;w)  + & \sum_{\alpha, \hat{y}_\alpha} b_\alpha(\hat{y}_\alpha) f_{(x,y),\alpha}(\hat{y}_\alpha;w)  + \epsilon \Big( \sum_i c_i H(b_i) + \sum_\alpha c_\alpha H(b_\alpha) \Big) \\ 
   %+ & \sum_{i,\alpha \in N(i), \hat{y}_i} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i) \Big(\sum_{\hat{y}_\alpha \setminus \hat{y}_i}b_\alpha(\hat{y}_\alpha) - b_i(\hat{y}_i) \Big) \nonumber
%\end{align}
%
%The dual function is obtained by 
%
%\begin{align}
  %\max_{b_i,b_\alpha }L(b_i,b_\alpha,\lambda;w) = & \sum_i \max_{b_i} \Bigg( \epsilon c_i H(b_i) + \sum_{\hat{y}_i}b_i(\hat{y}_i)\Big(f_{(x,y),i}(\hat{y}_i;w) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)  \Big) \Bigg)\\
 %+ & \sum_\alpha \max_{b_\alpha} \Bigg( \epsilon c_\alpha H(b_\alpha) + \sum_{\hat{y}_\alpha}b_\alpha(\hat{y}_\alpha)\Big(f_{(x,y),\alpha}(\hat{y}_\alpha;w) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)  \Big) \Bigg) \nonumber
%\end{align}

%Since log partition function is the conjugate dual of the entropy, we obtain the final approximation as follows.
%
%\begin{align}
  %\ln Z_{\epsilon}(x,y) \approx & \min_{\lambda_{(x,y),i \rightarrow \alpha (\hat{y}_i) }} \sum_{i} \epsilon c_i \ln \sum_{\hat{y}_i} \exp \frac{f_{(x,y),i}(\hat{y}_i;w) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i} \\
                       %+ &  \sum_{\alpha} \epsilon c_\alpha \ln \sum_{\hat{y}_\alpha} \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha;w) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha} 
%\end{align}

%Therefore, the structured prediction program (\ref{eqn:struct_pred_prog}) is approximated by
%
%\begin{align}
  %\label{eqn:struct_pred_prog_approx}
  %\min_{w, \lambda_{(x,y),i \rightarrow \alpha}} \sum_{(x,y) \in D} \Bigg( &\sum_{i} \epsilon c_i \ln \sum_{\hat{y}_i} \exp \frac{f_{(x,y),i}(\hat{y}_i;w) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i} \\
                       %+ &  \sum_{\alpha} \epsilon c_\alpha \ln \sum_{\hat{y}_\alpha} \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha;w) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha} \nonumber \\
                       %- & \sum_k \big(\sum_{k \in \mathcal{V}_k}f_{k,i}(x,y_i;w_k) + \sum_{\alpha \in \mathcal{E}_k} f_{k,\alpha}(x,y_\alpha;w_k)   \big)  \Bigg) \nonumber
%\end{align}
%
%To solve Equation \ref{eqn:struct_pred_prog_approx}, we use alternating minimization: minimizing $\lambda$ while fix $w$, and then minimize over $w$ while fix $\lambda$. We show more details below.

%\subsection{Alternating minimization}

%\subsubsection{block coordinate descent}

\begin{figure*}
%\vspace{-0.5cm}
\fbox{
\begin{minipage}[c]{13.7cm}
%{\bf Algorithm: Message Passing Inference} 

Repeat until convergence

\begin{enumerate}[labelindent=0pt,labelwidth=\widthof{\ref{last-item}},label=\arabic*.,itemindent=1em,leftmargin=!]
\item Iterate over $r$:
\bea
&&\hspace{-1.2cm}\forall p\in P(r), \hat y_r \nonumber\\
&&\hspace{-0.9cm} \mu_{p\rightarrow r}(\hat y_r) = \epsilon c_p \ln \sum_{\hat y_p\setminus \hat y_r} \exp \frac{f_p^\ell(\hat y_p) - \sum_{p^\prime\in P(p)}\lambda_{p\rightarrow p^\prime}(\hat y_p) + \sum_{r^\prime\in C(p)\setminus r} \lambda_{r^\prime\rightarrow p}(\hat y_{r^\prime})}{\epsilon c_p}\label{eq:MPMu}\\
%&&\hspace{-1.2cm}\forall p\in P(r), \hat y_r \nonumber\\
&&\hspace{-0.9cm} \lambda_{r\rightarrow p}(\hat y_r) \propto \frac{c_p}{c_r + \!\!\sum\limits_{p\in P(r)}\!\! c_p} \!\!\left(\!\!f_r^\ell(\hat y_r) + \sum_{c\in C(r)} \lambda_{c\rightarrow r}(\hat y_c) + \sum_{p\in P(r)} \mu_{p\rightarrow r}(\hat y_r)\!\!\right)\!\! - \mu_{p\rightarrow r}(\hat y_r)\label{eq:MPLambda}
\eea

\item Ensuring that the Armijo rule holds for stepsize $\eta$, update the parameter vector $w$ via\label{last-item}
\bes
w \leftarrow w - \eta\left(\sum_{(x,y),r,\hat y_r} b_{(x,y),r}(\hat y_r)\nabla_w f_r(x,\hat y_r;w) - \nabla_w \overline{F}(w)\right)
\ees

\end{enumerate}

\end{minipage}
}
\vspace{-0.3cm}
\caption{Our Nonlinear Structured Prediction Algorithm. %{\color{red} you haven't defined $\overline{F}$}
}
\label{fig:NonLinStructPredAlgo}
\end{figure*}

We next derive a message passing algorithm to optimize \equref{eq:structPredGeneralDual} using block-coordinate descent to alternate between computing the messages  and performing weight vector updates. We emphasize again that this is possible only if $\epsilon c_r \geq 0$ $\forall r$, 
as in that case  the Gibbs-Helmholtz free energy is convex everywhere. Strictly speaking, we require convexity only within the set of feasible beliefs $\C_{(x,y)}$. Hence it is possible to relax the non-negativity restriction of $\epsilon c_r \geq 0$ $\forall r$ slightly. %Indeed computation of the dual is possible in a slightly more general case, \ie, if the Gibbs-Helmholtz free energy is convex only within the domain of feasible beliefs $\C_{(x,y)}$.
However, we neglect this extension in the following. %{\color{red} this is very confusing, can you either elaborate and clarify or delete}

%Next we outline a block-coordinate descent scheme to optimize \equref{eq:structPredGeneralDual} using the following two operations: 
 \figref{fig:NonLinStructPredAlgo}  summarizes %\hfill$\blacksquare$
our  non-linear structured prediction algorithm.
Given a fixed $w$ in the first step,  we iterate through all regions $r$ and use block-coordinate descent to find the globally optimal value of \equref{eq:structPredGeneralDual} \wrt $\lambda_{(x,y),r \rightarrow p}(\hat y_r)$ $\forall \hat y_r, p\in P(r)$. This can be done  jointly in  closed form and therefore can be computed very efficiently. The second step employs the Armijo rule to find a stepsize along the negative gradient \wrt $w$ to ensure sufficient decrease. %Those two steps are more carefully defined in the following.

\begin{claim}
For a chosen region $r$, we let $\mu$ be defined as specified in \equref{eq:MPMu} of \figref{fig:NonLinStructPredAlgo}. The block-coordinate descent update of $\lambda_{r\rightarrow p}(\hat y_r)$ $\forall p\in P(r), \hat y_r$ is then analytically computed via
\equref{eq:MPLambda} to minimize the cost function in \equref{eq:structPredGeneralDual} \wrt the chosen block of variables. %{\color{red} If there is space, we should have the form of the things here I think}
\end{claim}
{\bf Proof:} The proof follows \cite{Schwing2013}.\hfill$\blacksquare$

The gradient of the cost function in \equref{eq:structPredGeneralDual} \wrt $w$ is given by
$\sum_{(x,y),r,\hat y_r} b_{(x,y),r}(\hat y_r)\nabla_w f_r(x,\hat y_r;w) - \nabla_w \overline{F}(w)$
which follows from a straightforward computation. The convergence properties for our algorithm are summarized in the following claim.
\begin{claim}
The block-coordinate descent algorithm defined in \figref{fig:NonLinStructPredAlgo} is guaranteed to monotonically decrease the cost function.
\end{claim}
{\bf Proof:}
%Block-coordinate descent schemes are guaranteed to converge if the cost function is convex while making sure that a sufficient descent is taken, \eg, via the Armijo rule.
When optimizing \wrt blocks of Lagrange multipliers $\lambda$ we ensure that the cost function decreases since we minimize a convex function analytically~\cite{Tseng1987}. Similarly via the Armijo rule we ensure that a descent step \wrt $w$ is taken, which concludes the proof. \hfill$\blacksquare$

In practice, Armijo line-search might be prohibitively expensive for larger models with millions of parameters. At the expense of loosing guarantees for monotonic decrease, it can be replaced with subgradient steps. % which are  more suitable if $F$ is not smooth. %Note that our approach has made no assumptions on  $F$. %, hence it is generally very hard to proof much more.
For non-smooth functions we found the latter to perform better in practice. Thus we employ  subgradient methods for our  experiments. % presented in the following. %{\color{red} say what we do in practice}

%The terms that are related to a node $i$ in the model $\lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)$ for every $\alpha \in N(i)$, every $\hat{y}_i$ and every $(x,y) \in D$ are:
%
%\begin{align}
  %\label{eqn:lambda_block}
  %\min_{\lambda_{(x,y),i \rightarrow \alpha}}  &\epsilon c_i \ln \sum_{\hat{y}_i} \exp \frac{f_{(x,y),i}(\hat{y}_i;w) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i} \\
                       %+ &  \sum_{\alpha} \epsilon c_\alpha \ln \sum_{\hat{y}_\alpha} \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha;w) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha} \nonumber 
%\end{align}
%
%Let
%\begin{align}
  %\mu_{(x,y),\alpha \rightarrow i}(\hat{y}_i) = \epsilon c_\alpha \ln \sum_{\hat{y}_\alpha \setminus \hat{y}_i} \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha;w) + \sum_{j \in N(\alpha) \setminus i} \lambda_{(x,y),j \rightarrow \alpha}(\hat{y}_j)}{\epsilon c_\alpha}
%\end{align}
%
%Then, Equation \ref{eqn:lambda_block} becomes:
%
%\begin{align}
  %\label{eqn:lambda_block_mu}
  %\min_{\lambda_{(x,y),i \rightarrow \alpha}}  & \epsilon c_i \ln \sum_{\hat{y}_i} \exp \frac{f_{(x,y),i}(\hat{y}_i;w) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i} \\
                       %+ &  \sum_{\alpha} \epsilon c_\alpha \ln \sum_{\hat{y}_\alpha} \exp \frac{\mu_{(x,y),\alpha \rightarrow i}(\hat{y}_i) + \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha} \nonumber 
%\end{align}
%
%The optimal $\lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)$ is obtained when the gradient vanishes: 
%
%\begin{align}
  %\lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i) \propto \frac{c_\alpha}{c_i+\sum_{\alpha \in N(i)}c_\alpha} \Bigg( f_{(x,y),i}(\hat{y}_i;w) + \sum_{\alpha \in N(i)}\mu_{(x,y),\alpha \rightarrow i}(\hat{y}_i) \Bigg) - \mu_{(x,y),\alpha \rightarrow i}(\hat{y}_i)
%\end{align}
%
%\subsubsection{Gradient descent}
%Recall, the structured prediction program is approximated by Equation \ref{eqn:struct_pred_prog_approx}
%
%\begin{align}
  %\min_{w, \lambda_{(x,y),i \rightarrow \alpha}} \sum_{(x,y) \in D} \Bigg( &\sum_{i} \epsilon c_i \ln \sum_{\hat{y}_i} \exp \frac{f_{(x,y),i}(\hat{y}_i;w) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i} \nonumber \\
                       %+ &  \sum_{\alpha} \epsilon c_\alpha \ln \sum_{\hat{y}_\alpha} \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha;w) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha} \nonumber \\
                       %- & \sum_k \big(\sum_{i \in \mathcal{V}_k}f_{k,i}(x,y_i;w_k) + \sum_{\alpha \in \mathcal{E}_k} f_{k,\alpha}(x,y_\alpha;w_k)   \big)  \Bigg) \nonumber
%\end{align}
%
%We minimize the program by changing $w$ in the direction of the negative gradient (i.e., gradient descent).
%
%Take derivative with respect to $w_k$, and then we have
%
%\begin{align}
  %\sum_{(x,y) \in D} \Bigg( & \sum_{i} \frac{\sum_{\hat{y}_i} \exp \frac{f_{(x,y),i}(\hat{y}_i) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i}}{\sum_{\hat{y}_{i'}} \exp \frac{f_{(x,y),i'}(\hat{y}_{i'}) - \sum_{\alpha \in N(i')} \lambda_{(x,y),i' \rightarrow \alpha}(\hat{y}_{i'})}{\epsilon c_i}} \cdot \frac{\partial f_{k,i}(x,\hat{y}_i;w_k)}{\partial w_k} \\
   %& \sum_{\alpha} \frac{\sum_{\hat{y}_\alpha} \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha}}{\sum_{\hat{y}_{\alpha'}} \exp \frac{f_{(x,y),\alpha'}(\hat{y}_{\alpha'}) + \sum_{i \in N(\alpha')} \lambda_{(x,y),i \rightarrow \alpha'}(\hat{y}_i)}{\epsilon c_\alpha}} \cdot \frac{\partial f_{k,\alpha}(x,\hat{y}_\alpha;w_k)}{\partial w_k} \nonumber \\
   %& - \Big( \sum_{i \in \mathcal{V}_k} \frac{\partial f_{k,i}(x,y_i;w_k)}{\partial w_k} + \sum_{\alpha \in \mathcal{E}_k} \frac{\partial f_{k,\alpha}(x,y_\alpha;w_k)}{\partial w_k} \Big) \Bigg) \nonumber 
%\end{align}
%
%This can be simplified to
%
%\begin{align}
 %\label{eqn:learn_w}
 %\sum_{(x,y) \in D} \Bigg( & \sum_{i,\hat{y}_i}b_i(\hat{y}_i) \frac{\partial f_{k,i}(x,\hat{y}_i;w_k)}{\partial w_k} + \sum_{\alpha,\hat{y}_\alpha}b_\alpha(\hat{y}_\alpha) \frac{\partial f_{k,\alpha}(x,\hat{y}_\alpha;w_k)}{\partial w_k} \\
   %& - \sum_{i \in \mathcal{V}_k}\frac{\partial f_{k,i}(x,y_i;w_k)}{\partial w_k} - \sum_{\alpha \in \mathcal{E}_k} \frac{\partial f_{k,\alpha}(x,y_\alpha;w_k)}{\partial w_k} \Bigg) \nonumber
%\end{align}
%
%where
%\begin{align}
  %b_i(\hat{y}_i) \propto \exp \frac{f_{(x,y),i}(\hat{y}_i) - \sum_{\alpha \in N(i)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_i} \nonumber \\
  %b_\alpha(\hat{y}_\alpha) \propto \exp \frac{f_{(x,y),\alpha}(\hat{y}_\alpha) + \sum_{i \in N(\alpha)} \lambda_{(x,y),i \rightarrow \alpha}(\hat{y}_i)}{\epsilon c_\alpha} \nonumber 
%\end{align}



 



==> resultsTables.tex <==
\subsection{Dataset Add1}
In this dataset, the second image is the frist image added by one.

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 61.07/78.10 & 62.78/79.18 & 62.29/78.89 & 62.11/78.74 & 62.16/78.75 \\
    \hline
    Model-RandInit                & 90.55/91.00 & 90.66/91.34 & 90.34/91.40 & 90.16/91.36 & 90.24/91.52 \\
    \hline
    Model-PwTrain                 & 93.35/93.45 & 93.53/93.74 & 92.74/93.37 & 92.36/93.19 & 91.94/93.15 \\
    \hline
    Model-JointTrain              & 92.08/92.41 & 92.60/93.32 & 91.69/92.94 & 91.26/92.73 & 90.69/92.56 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Add1 (MNIST variation) dataset.
}
  \label{table:add1_mnist}
    \vspace{-0.4cm}
\end{table}
 
\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 61.07/78.10 & 62.78/79.18 & 62.29/78.89 & 62.11/78.74 & 62.16/78.75 \\
    \hline
    Model-RandInit                & 90.57/90.62 & 90.33/90.46 & 90.37/90.62 & 90.29/90.60 & 90.24/90.59 \\
    \hline
    Model-PwTrain                 & 93.27/93.28 & 93.67/93.73 & 93.46/93.62 & 93.21/93.48 & 93.24/93.60 \\
    \hline
    Model-JointTrain              & 92.16/92.24 & 93.19/93.36 & 92.90/93.34 & 92.78/93.28 & 92.60/93.25 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Add1 (MNIST variation) dataset with Oracle feature. The unary is same as Table \ref{table:add1_mnist}.
}
  \label{table:add1_mnist_oracle_feature}
    \vspace{-0.4cm}
\end{table}

\begin{figure}[h]
  \centering
  \begin{tabular}{c c c}
    \includegraphics[height=0.19\linewidth]{fig/add1_mnist_u_weight_filter_256.jpg} &
    \includegraphics[height=0.19\linewidth]{fig/add1_mnist_p_weight_matrix_256.jpg} &
    \includegraphics[height=0.19\linewidth]{fig/add1_mnist_h256_trainingEnergy.jpg} \\
    Add1: Unary filters & Add1: Pairwise weights & Training Energy
  \end{tabular}
  \caption{The weights of our model learned from Add1 dataset. We show the case where the number of hindden units is 256. For pairwise weights, the more reddish, the larger the weight is, and the more blueish, the smaller the weight is (best viewed in color). }
  \label{fig:add1_filters}
\end{figure}



\subsection{Dataset PM1}
In this dataset, the sceond image is the first image added by one, minused by one, or have the same digit value.

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 61.12/78.13 & 62.82/79.23 & 62.48/78.98 & 62.78/79.15 & 62.36/78.95 \\
    \hline
    Model-RandInit                & 76.20/84.31 & 77.15/85.00 & 77.88/85.58 & 77.78/85.52 & 77.43/85.44 \\
    \hline
    Model-PwTrain                 & 78.07/86.14 & 79.25/86.83 & 79.01/86.70 & 79.01/86.65 & 78.79/86.53 \\
    \hline
    Model-JointTrain              & 77.90/85.62 & 79.26/86.61 & 78.94/86.54 & 78.90/86.49 & 78.44/86.34 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on PM1 (MNIST variation) dataset.
}
  \label{table:pm1_mnist}
    \vspace{-0.4cm}
\end{table}
 
\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 61.12/78.13 & 62.82/79.23 & 62.48/78.98 & 62.78/79.15 & 62.36/78.95 \\
    \hline
    Model-RandInit                & 76.10/84.04 & 77.64/84.92 & 78.18/85.44 & 78.47/85.57 & 78.21/85.40 \\
    \hline
    Model-PwTrain                 & 78.00/86.06 & 79.38/86.85 & 79.53/86.80 & 79.76/86.90 & 79.54/86.76 \\
    \hline
    Model-JointTrain              & 77.97/85.54 & 79.66/86.68 & 79.68/86.69 & 80.06/86.89 & 79.69/86.74 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on PM1 (MNIST variation) dataset with Oracle feature. The unary is same as Table \ref{table:pm1_mnist}.
}
  \label{table:pm1_mnist_oracle_feature}
    \vspace{-0.4cm}
\end{table}


\begin{figure}[h]
  \centering
  \begin{tabular}{c c c}
    \includegraphics[height=0.19\linewidth]{fig/pm1_mnist_u_weight_filter_256.jpg} &
    \includegraphics[height=0.19\linewidth]{fig/pm1_mnist_p_weight_matrix_256.jpg} &
    \includegraphics[height=0.19\linewidth]{fig/pm1_mnist_h512_trainingEnergy.jpg} \\
    PM1: Unary filters & PM1: Pairwise weights & Training Energy
  \end{tabular}
  \caption{The weights of our model learned from PM1 dataset. We show the case where the number of hindden units is 256. For pairwise weights, the more reddish, the larger the weight is, and the more blueish, the smaller the weight is (best viewed in color). }
  \label{fig:pm1_filters}
\end{figure}


\subsection{Dataset Big}
In this dataset, the second one digit is larger than or equal to the first digit.

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 59.33/77.02 & 61.83/78.61 & 61.30/78.41 & 61.64/78.56 & 61.23/78.24 \\
    \hline
    Model-RandInit                & 63.37/78.31 & 67.26/81.00 & 67.91/81.54 & 68.66/81.95 & 68.15/81.64 \\
    \hline
    Model-PwTrain                 & 66.46/80.70 & 68.97/82.29 & 68.75/82.14 & 68.56/82.02 & 68.23/81.84 \\
    \hline
    Model-JointTrain              & 67.22/81.03 & 69.46/82.49 & 68.91/82.16 & 68.84/82.19 & 68.55/82.01 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Big (MNIST variation) dataset.
}
  \label{table:big_mnist}
    \vspace{-0.4cm}
\end{table}
 
\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 59.33/77.02 & 61.83/78.61 & 61.30/78.41 & 61.64/78.56 & 61.23/78.24 \\
    \hline
    Model-RandInit                & 64.78/79.60 & 67.82/81.41 & 67.80/81.49 & 68.60/81.86 & 67.74/81.26 \\
    \hline
    Model-PwTrain                 & 65.74/80.42 & 68.70/82.19 & 68.53/82.06 & 68.67/82.12 & 68.64/82.07 \\
    \hline
    Model-JointTrain              & 67.11/81.03 & 69.18/82.41 & 69.22/82.41 & 69.22/82.38 & 69.04/82.27 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Big (MNIST variation) dataset with Oracle feature. The unary is same as Table \ref{table:big_mnist}.
}
  \label{table:big_mnist_oracle_feature}
    \vspace{-0.4cm}
\end{table}


\begin{figure}[h]
  \centering
  \begin{tabular}{c c c}
    \includegraphics[height=0.19\linewidth]{fig/big_mnist_u_weight_filter_256.jpg} &
    \includegraphics[height=0.19\linewidth]{fig/big_mnist_p_weight_matrix_256.jpg} &
    \includegraphics[height=0.19\linewidth]{fig/big_mnist_h256_trainingEnergy.jpg} \\
    Big: Unary filters & Big: Pairwise weights & Training Energy
  \end{tabular}
  \caption{The weights of our model learned from Big dataset. We show the case where the number of hindden units is 256. For pairwise weights, the more reddish, the larger the weight is, and the more blueish, the smaller the weight is (best viewed in color). }
  \label{fig:big_filters}
\end{figure}


\subsection{Dataset Word20}
In this dataset, we created variations of 20 English words. In Table \ref{table:word20_edge_dist1}, we showed the performance of our models with edges connecting neighboring characters only (i.e., 2-gram). In addition to 2-gram, we also tested our model with longer edge connection, which connects both neighboring characters and every other two characters (e.g., 1st character is connected to 2nd and 3rd character). The resutls are shown in Table \ref{table:word20_edge_dist2}. To further demonstrate that our method is capable of training deep models, we tested our models with 2-layer MLP with 2-gram connections. The number of hidden units in the first layer is fixed to be 512, and we varied the number of hidden units in the second layer from 16 to 512, as shown in Table \ref{table:word20_2layer}.

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 7.35/60.89 & 10.95/65.33 & 12.35/66.88 & 12.80/66.96 & 12.30/67.29 \\
    \hline
    Model-RandInit                & 42.85/77.60 & 50.45/81.09 & 56.50/84.64 & 59.10/85.52 & 60.35/86.12 \\
    \hline
    Model-PwTrain                 & 31.40/72.39 & 40.50/78.52 & 45.40/81.41 & 49.65/83.06 & 50.65/83.74 \\
    \hline
    Model-JointTrain              & 45.10/78.35 & 53.85/83.17 & 60.50/86.24 & 62.60/87.31 & 63.45/87.73 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Word20 dataset. Edges connect only neighboring characters.
}
  \label{table:word20_edge_dist1}
    \vspace{-0.4cm}
\end{table}

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 7.35/60.89 & 10.95/65.33 & 12.35/66.88 & 12.80/66.96 & 12.30/67.29 \\
    \hline
    Model-RandInit                & 47.95/72.74 & 55.50/77.54 & 49.00/70.78 & 52.15/74.59 & 54.25/76.68 \\
    \hline
    Model-PwTrain                 & 50.45/83.85 & 64.10/89.21 & 71.85/91.75 & 75.75/93.01 & 78.20/93.74 \\
    \hline
    Model-JointTrain              & 60.25/81.08 & 69.60/86.14 & 75.25/89.17 & 78.00/90.80 & 78.50/91.21 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Word20 dataset. Edges connect both neighboring characters and distance-2 characters. The unary is the same as Table \ref{table:word20_edge_dist1}.
}
  \label{table:word20_edge_dist2}
    \vspace{-0.4cm}
\end{table}

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h2-32 & h2-64 & h2-128 & h2-256 & h2-512 \\
    \hline
    \hline
    Unary only                    & 14.30/69.15 & 16.55/70.96 & 18.50/72.11 & 17.35/71.70 & 18.80/72.24 \\
    \hline
    Model-RandInit                & 65.80/88.74 & 70.65/90.73 & 69.80/90.26 & 69.05/89.76 & 68.60/89.70 \\
    \hline
    Model-PwTrain                 & 63.60/88.99 & 66.40/90.02 & 69.95/91.02 & 71.00/91.43 & 71.60/91.92 \\
    \hline
    Model-JointTrain              & 70.45/90.66 & 71.40/91.03 & 72.95/91.65 & 73.20/91.72 & 72.20/91.87 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Word20 dataset. The classifier for the unary potential is a 2-layer MLP with first layer fixed to be 512 ReLU units. We tested the pefromance with various number of hidden units in the second layer.
}
  \label{table:word20_2layer}
    \vspace{-0.4cm}
\end{table}


\begin{figure}[h]
  \centering
  \begin{tabular}{c c c c}
    \includegraphics[height=0.18\linewidth]{fig/1x5word20_u_weight_filter_256.jpg} &
    \includegraphics[height=0.18\linewidth]{fig/1x5word20_p_weight_matrix_256.jpg} &
    \includegraphics[height=0.18\linewidth]{fig/1x5word20_p_weight_matrix2_256.jpg} &
    \includegraphics[height=0.18\linewidth]{fig/1x5word20_h256_trainingEnergy.jpg}  \\
    Word20: Unary filters & Word20: 2-gram & Word20: distance-2 edges & Training Energy
  \end{tabular}
  \caption{The weights of our model learned from Word20 dataset. We show the case where the number of hindden units is 256. For pairwise weights, the more reddish, the larger the weight is, and the more blueish, the smaller the weight is (best viewed in color). }
  \label{fig:word20_filters}
\end{figure}

\begin{figure}[h]
  \centering
  \begin{tabular}{c c c c}
    \includegraphics[height=0.18\linewidth]{fig/1x5word50_u_weight_filter_256.jpg} &
    \includegraphics[height=0.18\linewidth]{fig/1x5word50_p_weight_matrix_256.jpg} &
    \includegraphics[height=0.18\linewidth]{fig/1x5word50_p_weight_matrix2_256.jpg} &
    \includegraphics[height=0.18\linewidth]{fig/1x5word50_h256_trainingEnergy.jpg}  \\
    Word50: Unary filters & Word50: 2-gram & Word50: distance-2 edges & Training Energy
  \end{tabular}
  \caption{The weights of our model learned from Word50 datasets. We show the case where the number of hindden units is 256.  For pairwise weights, the more reddish, the larger the weight is, and the more blueish, the smaller the weight is (best viewed in color). Note that the edge weights learned from Word50 dataset are more complicate than Word20 dataset.}
  \label{fig:word50_filters}
\end{figure}


\subsection{Dataset Word50}
Herein, we tested our model on more complex datasets with 50 English words. We conducted three similar experiments as Word20. In Table \ref{table:word50_edge_dist1}, we showed the performance of our models with edges connecting neighboring characters only (i.e., 2-gram). In addition to 2-gram, we also tested our model with longer edge connection, which connects every other two characters (e.g., 1st character is connected to 3rd character). The resutls are shown in Table \ref{table:word50_edge_dist2}. To further demonstrate that our method is capable of training deep models, we tested our models with 2-layer MLP with 2-gram connections. The number of hidden units in the first layer is fixed to be 512, and we varied the number of hidden units in the second layer from 16 to 512, as shown in Table \ref{table:word50_2layer}.

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 8.45/61.10  & 11.10/64.34 & 12.40/66.29 & 12.30/66.65 & 13.75/66.88 \\
    \hline
    Model-RandInit                & 17.35/64.49 & 22.75/69.03 & 30.75/74.70 & 33.10/75.89 & 35.05/77.29 \\
    \hline
    Model-PwTrain                 & 11.85/63.09 & 16.90/67.94 & 23.60/72.04 & 24.90/72.63 & 25.35/73.42 \\
    \hline
    Model-JointTrain              & 19.45/66.27 & 26.85/72.03 & 31.25/75.63 & 34.15/77.23 & 36.65/78.61 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Word50 dataset. Edges connect only neighboring characters.
}
  \label{table:word50_edge_dist1}
    \vspace{-0.4cm}
\end{table}

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h-128 & h-256 & h-512 & h-768 & h-1024 \\
    \hline
    \hline
    Unary only                    & 8.45/61.10  & 11.10/64.34 & 12.40/66.29 & 12.30/66.65 & 13.75/66.88 \\
    \hline
    Model-RandInit                & 19.30/62.05 & 27.50/68.23 & 35.20/73.52 & 39.50/75.94 & 41.80/77.15 \\
    \hline
    Model-PwTrain                 & 8.00/57.07  & 13.95/63.14 & 19.00/68.22 & 20.50/69.93 & 22.55/71.64 \\
    \hline
    Model-JointTrain              & 23.15/65.66 & 31.95/71.45 & 38.85/76.49 & 42.00/78.18 & 44.60/79.46 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Word50 dataset. Edges connect both neighboring characters and distance-2 characters. The unary is the same as Table \ref{table:word50_edge_dist1}.
}
  \label{table:word50_edge_dist2}
    \vspace{-0.4cm}
\end{table}

\begin{table}[h]
  \centering
  \scalebox{0.88}{
   \addtolength{\tabcolsep}{-1.11pt}
   \hspace{-1.3mm}\begin{tabular}{| l | c | c | c | c | c |}
%    \hline
%    \hline
%    \multicolumn{7}{c}{Incremental effect}  \\
%    \hline
    \hline
    Model & h2-32 & h2-64 & h2-128 & h2-256 & h2-512 \\
    \hline
    \hline
    Unary only                    & 15.10/68.32 & 17.75/71.09 & 20.15/71.92 & 18.95/72.11 & 19.85/72.20 \\
    \hline
    Model-RandInit                & 38.50/78.75 & 44.70/81.85 & 44.90/81.86 & 46.25/82.61 & 45.50/82.56 \\
    \hline
    Model-PwTrain                 & 35.60/78.76 & 39.65/81.48 & 42.50/82.45 & 43.35/83.06 & 44.00/83.12 \\
    \hline
    Model-JointTrain              & 42.55/81.42 & 45.60/83.30 & 47.55/83.71 & 46.55/83.75 & 47.00/84.07 \\
    \hline
  \end{tabular} 
  }
  \caption{ Word Accuracy / Character Accuracy on Word50 dataset. The classifier for the unary potential is a 2-layer MLP with first layer fixed to be 512 ReLU units. We tested the pefromance with various number of hidden units in the second layer.
}
  \label{table:word50_2layer}
    \vspace{-0.4cm}
\end{table}
